UNOC: Understanding Occlusion for Embodied Presence in Virtual Reality

Tracking body and hand motions in the 3D space is essential for social and self-presence in augmented and virtual environments. Unlike the popular 3D pose estimation setting, the problem is often formulated as inside-out tracking based on embodied perception (e.g., egocentric cameras, handheld sensors). In this paper, we propose a new data-driven framework for inside-out body tracking, targeting challenges of omnipresent occlusions in optimization-based methods (e.g., inverse kinematics solvers). We first collect a large-scale motion capture dataset with both body and finger motions using optical markers and inertial sensors. This dataset focuses on social scenarios and captures ground truth poses under self-occlusions and body-hand interactions. We then simulate the occlusion patterns in head-mounted camera views on the captured ground truth using a ray casting algorithm and learn a deep neural network to infer the occluded body parts. In the experiments, we show that our method is able to generate high-fidelity embodied poses by applying the proposed method on the task of real-time inside-out body tracking, finger motion synthesis, and 3-point inverse kinematics.

==> abstract.tex <==
\begin{abstract}

%% Background
Tracking body and hand motions in the 3D space is essential for social and self-presence in augmented and virtual environments. Unlike the popular 3D pose estimation setting, the problem is often formulated as inside-out tracking based on embodied perception (\eg, egocentric cameras, handheld sensors).
%% Method Overview
In this paper, we propose a new data-driven framework for inside-out body tracking, targeting challenges of omnipresent occlusions in optimization-based methods (\eg, inverse kinematics solvers).
We first collect a large-scale Mocap dataset with both body and finger motions using optical markers and inertial sensors. This dataset focuses on  social scenarios and captures groundtruth poses under self-occlusions and body-hand interactions.
We then simulate the occlusion patterns in head-mounted camera views on the captured groundtruth using a ray casting algorithm and learn a deep neural network to infer the occluded body parts.
% In the experiments, we apply the proposed method on the task of real-time inside-out body tracking and show our method is able to generate high-fidelity embodied poses.
In the experiments, we show that our method is able to generate high-fidelity embodied poses by applying the proposed method on the task of real-time inside-out body tracking, finger motion synthesis, and 3-point inverse kinematics.

% Inside-out tracking based on head-mounted cameras is critical for virtual and augmented reality. Besides headsets and hands tracking, inside-out body tracking, which is essential for social and self-presence in virtual and augmented environments, remains an under-explored challenge due to the omnipresent visual occlusion of the body parts and the lack of sufficient data to address occlusion.
% We propose a dataset with both body and finger motions targeted at everyday poses in social meetings, with frequent occlusion through interactions between hands, arms, and other body parts.The dataset consists of 1.8M frames of body and hand tracking in 237 sequences, with seated and standing poses, scripted and unscripted gestures. We formulate a new problem for body tracking in which tracked joints are subject to severe occlusions with views from head-mounted cameras. We propose a novel temporal neural network for recovering body and finger poses from visible joints to tackle the frequent intermittent occlusions.
% We show how the proposed dataset and network contribute to solving the problem of real-time inside-out body tracking.

% with devices moving from tethered to all-in-one mobile solutions.
 %based on inverse kinematics loss and XXX (skip connections?) to leverage information from the past to tackle the frequent intermittent occlusions.

% Inside-out body tracking is becoming increasingly important with head-mounted virtual and augmented reality devices moving from tethered solutions to all-in-one mobile devices.
% Virtual environments can create a natural feeling of being socially present when participants share the same virtual room and have realistically animated avatars.
% Using inside-out body tracking with head-mounted cameras, visual occlusion is omnipresent, especially for the lower body.
% We propose a dataset specifically designed for everyday poses in social meetings, with frequent hand-body and arm-arm interaction. % and self occlusions.
% The dataset consists of 1.8M frames of body and hand tracking in 237 sequences, with seated and standing poses, scripted as well as unscripted gestures.
% We show that our dataset adds unique motions to the pool of existing collections and that we can create a model to fill in missing pose information with it.

% In this paper, we propose a model which fills in missing information when body parts are occluded; creating a natural looking pose even when body parts are untracked for many seconds.
% We created a unique motion capture dataset for this task, which is specifically designed for difficult to track poses that happen frequently during conversations and meetings.

\end{abstract}

==> impact.tex <==
\section{Broader Impact}

% In this paper, we propose a data-driven approach for handling occlusions in embodied presence in augmented and virtual reality. To our best knowledge, this is the first paper targets this important yet under-studied application.
We propose a data-driven approach for handling occlusions in embodied presence for augmented and virtual reality. To the best of our knowledge, this is the first paper targeting this important yet under-studied application.
Accurately tracked body movement and finger motions complement verbal communication and facial expression. They provide a more convincing experience of self and social presence in a virtually connected space, which is especially important when families, friends, and colleagues are physically distant.  Furthermore virtual reality has been shown to increase empathy~\cite{empathy}, which could be important for e.g. jury trials~\cite{zoomJury}.

We should note, however, that our dataset was collected in a single facility embedded in a so-called WEIRD (Western, educated, industrialized, rich and democratic) society.  It is important to broaden the data to include a wider variety of ages, cultures, and people with disabilities (such as missing limbs).  Gestures are often culture-specific, which could lead to miscommunication if models do not generalize across wider populations.   Furthermore, properly evaluating the quality of interactions requires collaborating with other disciplines including social scientists, cultural experts, and broader communities.
